IKT-BT: Indirect Knowledge Transfer Behavior Tree Framework for Multi-Robot Systems Through Communication Eavesdropping

Multi-agent and multi-robot systems (MRS) often rely on direct communication for information sharing. This work explores an alternative approach inspired by eavesdropping mechanisms in nature that involves casual observation of agent interactions to enhance decentralized knowledge dissemination. We achieve this through a novel IKT-BT framework tailored for a behavior-based MRS, encapsulating knowledge and control actions in Behavior Trees (BT). We present two new BT-based modalities - eavesdrop-update (EU) and eavesdrop-buffer-update (EBU) - incorporating unique eavesdropping strategies and efficient episodic memory management suited for resource-limited swarm robots. We theoretically analyze the IKT-BT framework for an MRS and validate the performance of the proposed modalities through extensive experiments simulating a search and rescue mission. Our results reveal improvements in both global mission performance outcomes and agent-level knowledge dissemination with a reduced need for direct communication.

==> OtherText.tex <==
%For the current study, we investigate direct and indirect knowledge transfer, and memory buffer priority transfer modalities and present a comparison between them to understand their effect on interaction rates and memory. 

In a direct query-response process, the robot facing an unknown condition broadcasts a request to its neighbors and awaits a response. Robots that have knowledge of the request respond by transferring the appropriate knowledge to the requesting robot. On the other hand, the indirect transfer involves a third robot overhearing/ eavesdropping on the query-response process between any two robots and utilizes the knowledge acquired in updating its own knowledge base $\mathcal{T}_{K}$ either immediately or by storing the messages in a timed buffer $Q_{tb}$ and using them later. 

We categorize the first variant of indirect knowledge transfer as \textit{eavesdrop-update} (EU) modality and the second variant as \textit{eavesdrop-buffer-update} (EBU) modality. The EBU modality is subtly different from the EU modality in how the knowledge is updated during indirect transfer. In the indirect knowledge transfer with immediate updates, the knowledge that is indirectly acquired is immediately merged with the existing knowledge base $\mathcal{T}_{K}$ of the robot. 

On the other hand, in the buffer variant (EBU), the messages are first stored in a timed buffer $Q_{tb}$ and retrieved only when the conditions corresponding to the stored message arise during a mission.  Further, the buffer $Q_{tb}$ is timed and has a fixed size which introduces an inherent priority sequence of knowledge by removing the messages that are not utilized beyond a time limit, during a mission. Figure \ref{fig:passiveLearn} summarizes these three modalities along with a \textit{query-response} modality that involves query and response operations without knowledge update.


The EU and EBU modalities can be structured as behavior trees $\mathcal{T}_{EU}$ and $\mathcal{T}_{EBU}$ respectively and can be combined with the primary tree $\mathcal{T}_{kt}$ as follows
\begin{align}
    \mathcal{T}_{kt}=Parallel(\mathcal{T}_{Control}&,\mathcal{T}_{Teach}, \nonumber \\
                                & Selector(\mathcal{T}_{EU/EBU},\mathcal{T}_{Learn}))
    \label{eq:kt}
\end{align}
by this combination, the selector applied ensures direct knowledge transfer (i.e \textit{query-response-update} or \textit{query-response-update})  as a fallback modality when indirect knowledge transfer fails. We present a generic BT structure for $\mathcal{T}_{EU}$ and $\mathcal{T}_{EBU}$ in figures \ref{fig:TEU} and \ref{fig:TEBU} respectively, and the indirect knowledge transfer algorithm \ref{alg:BTT} and \ref{alg:IKT-BT} that details the indirect knowledge transfer strategies.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/TEU.png}
    \caption{Behavior tree $\mathcal{T}_{EU}$ representing \textit{eavesdrop - update} modality}
    \label{fig:TEU}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/TEBU.png}
    \caption{Behavior tree $\mathcal{T}_{EBU}$ representing \textit{eavesdrop - buffer - update} modality}
    \label{fig:TEBU}
\end{figure}

\begin{algorithm}[h]
\caption{Function $\textbf{BTT} (inx,s_q)$}
\label{alg:BTT}
\begin{algorithmic}
\State \textbf{Input:} {$inx \leftarrow$ index, $s_q\leftarrow$ Condition Sequence}
\State \textbf{Data:} { $Q_{tb}\leftarrow$ Message Buffer, $\mathcal{T}_{Control}$, $L_{ks}$, $L_{ka}$,$L_{tb}$}
\State \textbf{Result:} {Merges a sub-tree $\mathcal{T}_k = Sequence (s_q, \mathcal{T}_{ka}^*)$ with control sub-tree $\mathcal{T}_{Control}.$}

           \State{$\mathcal{T}_{ka}^* \gets Q_{tb}(inx).response$}
            \State{$\mathcal{T}_k = Sequence (sq, \mathcal{T}_{ka}^*)$}
            \State{$\mathcal{T}_{Control} = Merge (\mathcal{T}_{Control}, \mathcal{T}_{k})$}
            \State{$Q_{tb}.RemoveAt(inx)$}
            \State{$L_{tb}.RemoveAt(inx)$}
            \State{$L_{ks}.add(s_q)$}
            \State{$L_{ka}.add(\mathcal{T}_{ka}^*)$}
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[h]
\caption{Indirect Knowledge Transfer \textbf{IKT-BT}.}
\label{alg:IKT-BT}
\begin{algorithmic}
\State \textbf{Input:} {$Q_m \leftarrow$ Eavesdropped messages list, $t_{b} \leftarrow$ Timeout for buffer,$L_{tb} \leftarrow$ list of buffer timers, $s_q \leftarrow$ Unknown condition}

\State \textbf{Data:} { $Q_{tb}\leftarrow$ Message Buffer, $\mathcal{T}_{Control}$, $L_{ks}$, $L_{ka}$}
\State \textbf{Result:} {Merges a sub-tree $\mathcal{T}_k = Sequence (s_q, \mathcal{T}_{ka}^*)$ with control sub-tree $\mathcal{T}_{Control}.$}
%\algnewcommand{\LeftComment}[1]{\Statex \(\triangleright\) #1}

\If{BufferMode}
\If{$Q_m.length()\neq 0$}
    \State{$ql \gets Q_m.length()$}
    \For {$i \gets 1$ to ql}
    \State {$Q_{tb}.Add(Q_m.pop())$}
    \State{$L_{tb}(i) \gets t_b$}
    \State{$ql \gets Q_m.length()$}
    \EndFor
    \If{$s_q$ not in $L_{ks}$}
        \For {$j \gets 1$ to $Q_{tb}.length()$}
        \If{$s_q = Q_{tb}(j).query$}
            \State{$BTT(j,s_q)$)}
            \State{\textbf{return} success}
        \EndIf
        \EndFor
    \EndIf
    \For {$k \gets 1$ to $L_{tb}.Length()$}
        \If{$L_{tb}(k)=0$}
            $Q_{tb}.RemoveAt(k)$
        \EndIf

    \EndFor

\EndIf
\Else{}
    \State{$ql \gets Q_m.length()$}
    \For {$i \gets 1$ to ql}
        \State{$s_q \gets Q_m(i).query$}
        \State{$BTT(i,s_q)$}
        \State{\textbf{return} success}
    \EndFor
\EndIf

\end{algorithmic}
\end{algorithm}








\subsection{Formalization of Indirect Knowledge Transfer}
The goal of the indirect knowledge transfer strategy is to have the high-level knowledge shared across multiple robots with indirect interactions like eavesdropping. In this section, we present the definitions of direct and indirect knowledge transfer and prove the knowledge transfer efficiency in indirect knowledge transfer called IKT-BTs.

First, we formalize the query possibilities in direct knowledge transfer modalities through the following lemma.

\begin{lemma}[\textbf{Interactions in direct knowledge transfer}]{\textit{ Among the two direct knowledge transfer modalities, the \textit{query-response-update} modality requires lesser interactions than \textit{query-response}. }
i.e., in an group of size $P$, a robot $i$ with knowledge of a condition sequence $s_c$ and with corresponding knowledge $\mathcal{T}_{k}^c$ can teach any robot $j$ that queries for condition sequence $s_c$. However, for robot $j$, when using \textit{query-response} modality, $s_c \notin K_{ks}$ and hence, $\mathcal{T}_{k}^c \notin \mathcal{T}_{K}$. Or otherwise, the robot $j$, never acquires knowledge  $\mathcal{T}_{k}^c$.
Hence, if there are multiple occurrences of $s_c$, i.e. if $n(s_c)\geq1$, the number of query requests $n(Queries)=n(s_c)$. So, the robot queries every time the condition is faced, in contrast to \textit{query-response-update}, where the knowledge is recorded and utilized for future purposes.




in a \textit{query-response} $\forall$ queries $s_q$, the knowledge 

Hence, \textit{query-response-update} has a more efficient process than 


Given an agent i, with $\mathcal{T}_{control_i}$,$\mathcal{T}_{teach_i}$ and $\mathcal{T}_{RL_i}$ as the sub-trees running in parallel according to definition 1. If $\exists$ a condition $Con_{current_i}$} s.t $Con_{current_i}\notin Conc_{i}$, and $\exists$ at least one agent $v$ in its communication range at time $t\in (0,\infty]$, s.t $Con_{current_i} \in Conc_k$. Then as the agent $i$ faces conditions $Con_{current_i}$ at time $t$, then $Con_{current_i} \in Conc_i$, and $\mathcal{T}_{ka}\subset\mathcal{T}_{control}$.

\textit{Proof.} Lets assume that the agent \textit{i} and \textit{k} have infinite communication ranges. As agent \textit{i} faces condition $Con_{current_i}$, the $\mathcal{T}_{RL}$ tree verifies the condition is not in agent \textit{i's}, $Conc_i$, and hence broadcasts a query. As, the query is received by agent \textit{k}, the $\mathcal{T}_{teach}$ verifies in it's known condition list $Conc_k$ and transmits the sub-tree $\mathcal{T}_{ka}$ in response. Agent $i$, merges this tree with the $\mathcal{T}_{control}$ tree and adds the condition $Con_{current_i}$it to the $Conc_i$ list.

We expand the above lemma to all the agents in the group through the following lemma.
\begin{lemma}
\textit{If $\exists$ a one and only agent k that has the knowledge tree $\mathcal{T}_{ka}$ for condition $Con_{current_k}$ in a group $G_{agents}$ of population $n(G_{agents})=P$. As time $t\rightarrow \infty$,}
\begin{center}
    $\forall G_i \in G_{agents}, Con_{current_k} \subset Conc_i, i= 1 \dots P$
\end{center}

\end{lemma}
\textit{Proof.} Lets assume that all the agents \textit{i} and \textit{k} are in the range of communication, and agent \textit{i} faces condition $Con_{current_i} \notin Conc_i$, also $Con_{current_i} \in Conc_k$. By lemma 1, $Con_{current_i} \in Conc_i$. This can also be proven to any agent \textit{j} within the communication range of \textit{i} or \textit{k}. Through one-to-one transmission of information after a sufficient amount of time, the sub-tree $\mathcal{T}_{ka}$ related to the condition $Con_{current_k}$ in known to all the agents under group. 
\end{lemma}
\begin{lemma}If $\exists$ a one and only agent k that has the knowledge tree $\mathcal{T}_{ka}$ for condition $Con_{current_k}$ in a group $G_{agents}$ of population $n(G_{agents})=P$. The minimum number of queries posted in regular learning is P-1 for the knowledge to be shared across all the agents. 
\end{lemma}
\textit{Proof.} For a minimum criterion, let us assume that all the robots are with in each other's communication range, and cool down times are set to zero. From lemma 1 and 2, in regular learning each agent posts a query once as the condition once learnt is added to its known conditions list. And hence, in the beginning as $P-1$ agents don't have information, a total of $P-1$ queries are posted in total.

\begin{lemma}
In ephemeral learning if the forgetfulness timer, $t_{e}\rightarrow \infty$, $\mathcal{T}_{EL}\rightarrow\mathcal{T}_{RL}$
\end{lemma}
\textit{Proof.} From the definition 4.2, 
\begin{center}
    $\mathcal{T}_{EL} = Parallel(\mathcal{T}_{RL},\mathcal{T}_{forget})$
\end{center}
As $t_{e} \rightarrow \infty$, from Algorithm 3, $\mathcal{T}_{forget}$ always returns \textit{Running} and hence $\mathcal{T}_{control})$ is never reset. So, an ephemeral learning tree at infinite forgetfulness timer behaves like a regular learner.

\begin{lemma}
The number of updates of $\mathcal{T}_{control}$ in $\mathcal{T}_{PL} \leqq \mathcal{T}_{APL}$
\end{lemma}

\textit{Proof.} To prove this, let us assume a set $Con$ with all possible conditions in a given scenario. i.e., any $Con_{current_i}\in Con \& Conc_i \subseteqq Con $. Where \textit{i} is agent index in a group of P agents. Let us assume an infinite communication range. At this point any robot can eavesdrop any communication happening between any two robots. Let, an agent \textit{a} query agent \textit{b} and an agent \textit{k} eavesdrop the communication and learn through PL. The condition under query is $Con_{current_a}$ and $Con_{current_a}\in Con_{current_b}$. With agent \textit{k} eaves dropping, from definitions 1 and 4.3, 
\begin{center}
    $Con_{current_a} \in Con_{current_a}$\\
    $Con_{current_a} \in ComsBuffer \Rightarrow Con_{current_a} \in Conc_k$
\end{center}
 The knowledge tree $\mathcal{T}_{ka}$ is updated across a, b and k. 
 On the other hand, when agents a, b and k learn through APL, from the definitions 1 and 4.4, 
 \begin{center}
  $Con_{current_a} \in Con_{current_a}$\\
  $Con_{current_a} \in ComsBuffer \Rightarrow Con_{current_a} \notin Conc_k$
 \end{center}
 If the agent \textit{k} does not face the condition $Con_{current_a}$ during the mission, $Conc_k$ never includes it and hence, the sub-tree $\mathcal{T}_{control}$ is never updated. And thus limiting the total number of updates for APL always less than or equal to updates in PL.
